On the calibration of Just-in-time Defect Prediction

Just in time defect prediction (JIT DP) leverages ML to identify defect-prone code commits, enabling quality assurance (QA) teams to allocate resources more efficiently by focusing on commits that are most likely to contain defects. Although JIT DP techniques have introduced improvements in terms of predictive accuracy, they are still susceptible to misclassification errors such as false positives and negatives. This can lead to wasted resources or undetected defects, a particularly critical concern when QA resources are limited. To mitigate these challenges and preserve the practical utility of JIT DP tools, it becomes essential to estimate the reliability of the predictions, i.e., computing confidence scores. Such scores can help practitioners determine the trustworthiness of predictions and thus prioritize them efficiently. A simple approach to computing confidence scores is to extract, alongside each prediction, the corresponding prediction probabilities and use them as indicators of confidence. However, for these probabilities to reliably serve as confidence scores, the predictive model must be well-calibrated. This means that the prediction probabilities must accurately represent the true likelihood of each prediction being correct. Miscalibration, common in modern ML models, distorts probability scores such that they do not align with the actual correctness probability. In this study, we evaluate the calibration of three JIT DP techniques to determine whether and to what extent they exhibit poor calibration. Furthermore, we assess whether post-calibration methods can improve the calibration of existing JIT defect prediction models. Our results reveal that all evaluated JIT DP models exhibit some level of miscalibration, with ECE ranging from 2-35%. Furthermore, post-calibration methods do not consistently improve the calibration.

==> tables/calibrated_CodeBERT4JIT.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{1pt}
\begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
        \multicolumn{6}{|c|}{Platt scaled CodeBERT4JIT with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT)} & {0.1778} &  {0.0269} & {0.5808} & {0.0854} & {0.0611} \\
        {Val. Min-Max} & {0.07-0.0.38} & {0.01-0.05} & {0.15-0.95} & {0.02-0.15} & {0.05-0.07} \\
        \hline
        Test (QT) & 0.1565 & 0.0238 & 0.5293 & 0.0894 & 0.0609 \\
        %\hline
        %\multicolumn{6}{|c|}{CodeBERT4JIT with QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS)} & {0.1355} &  {0.0425} & {0.4770} & {0.1139} & 0.0970 \\
        {Val. Min-Max} & {0.04-0.27} & {0.02-0.04} & {0.07-0.83} & {0.05-0.19} & {0.08-0.11} \\
        \hline
        Test (OS) & 0.1416 & 0.0425 & 0.4880 & 0.1361 & 0.09887 \\
        \hline
        \multicolumn{6}{|c|}{Temp. scaled CodeBERT4JIT with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS)} & {0.2127} & {0.0611} & {0.6387} & {0.3132} & {0.1059} \\
        {Val. Min-Max} & {0.12-0.3} & {0.03-0.15} & {0.29-0.95} & {0.09-0.54} & {0.09-0.14} \\
        \hline
        Test (OS) & 0.2092 & 0.0577 & 0.6437 & 0.3017 & 0.1063 \\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT)} & {0.2545} &  {0.0402} & {0.7324} & {0.2526} & {0.0672} \\
        {Val. Min-Max} & {0.11-0.35}  & {0.02-0.1} & {0.33-0.97} & {0.05-0.25} & {0.05-0.1} \\    
        \hline
        Test (QT) & 0.2404 & 0.0360 & 0.6693 & 0.2619 & 0.0669 \\
        \hline
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Calibrated CodeBERT4JIT QT and OPENSTACK}
    \label{calibrated_CodeBERT}
\end{table}

==> tables/calibrated_DeepJIT.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{1pt}
\begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
        \multicolumn{6}{|c|}{Platt scaled DeepJIT with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS)} & {0.0218} &  {0.0284} & {0.2433} &  {0.0901} & {0.0983}\\
        {Val. Min-Max} & {0.01-0.03}  & {0.02-0.04} & {0.09-0.59} & {0.04-0.14} & {0.08-0.10} \\
        \hline
        Test (OS)& 0.0236 & 0.0267  & 0.1693  & 0.0743 & 0.1002\\
        %\hline
        %\multicolumn{6}{|c|}{DeepJIT with QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT)} & {0.0153} &  {0.0159} & {0.3976} &  {0.0555} & {0.0585}\\
        {Val. Min-Max} & {0.01-0.02}  & {0.01-0.02} & {0.13-0.60} & {0.02-0.09} & {0.05-0.06} \\
        \hline
        Test (QT) & 0.0136 & 0.0190  & 0.1954  & 0.0844 & 0.0618\\
        \hline
        \multicolumn{6}{|c|}{Temp. scaled DeepJIT with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS)} & {0.3512} &  {0.3512} & {0.5119} &  {0.5094} & {0.2334}\\
        {Val. folds Min} & {0.32-0.38}  & {0.32-0.38} & {0.43-0.58} & {0.46-0.56}& {0.21-0.25} \\
        \hline
        Test (OS)& 0.3565 & 0.3565  & 0.5737  & 0.4973 & 0.2377\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT)} & {0.3436} &  {0.3436} & {0.6443} &  {0.5477} & {0.1927}\\
        {Val. folds Min} & {0.33-0.35}  & {0.33-0.35} & {0.52-0.93} & {0.52-0.57} & {0.18-0.20} \\    
        \hline
        Test (QT)& 0.3526 & 0.3526  & 0.5953  & 0.5814 & 0.2038\\
        \hline
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Calibrated DeepJIT QT and OPENSTACK}
    \label{calibrated_deepJIT}
\end{table}

==> tables/calibrated_LApredict.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{1pt}
\begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
        \multicolumn{6}{|c|}{Platt scaled LApredict with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS) DONE} & {0.2287} &  {0.1042} & {0.5715} & {0.2258} & {0.1912} \\
        {Val. Min-Max DONE} & {0.16-0.32} & {0.09-0.11} & {0.35-0.84} & {0.18-0.27} & {0.19-0.19} \\
        \hline
        Test (OS) DONE & 0.0880 & 0.0879 & 0.2759 & 0.2049 & 0.1480 \\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT) DONE} & {0.1985} &  {0.1038} & {0.5505} &  {0.2154} & {0.2053} \\
        {Val. Min-Max DONE} & {0.13-0.28}  & {0.09-0.11} & {0.35-0.87} & {0.19-0.25} & {0.2-0.21} \\
        \hline
        Test (QT) DONE & 0.3295 & 0.1452 & 0.7740 & 0.2644 & 0.1463 \\
        \hline
        \multicolumn{6}{|c|}{Temp. scaled LApredict with OPENSTACK \& QT}\\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (OS) DONE} & {0.2287} &  {0.1042} & {0.5715} &  {0.2258} & {0.1912} \\
        {Val. folds Min DONE} & {0.16-0.32}  & {0.09-0.11} & {0.35-0.84} & {0.18-0.26}& {0.19-0.19} \\
        \hline
        Test (OS) DONE & 0.0880 & 0.0879  & 0.2759 & 0.2049 & 0.1480 \\
        \hline
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. Avg (QT) DONE} & {0.1985} &  {0.1038} & {0.5505} &  {0.2154} & {0.2053} \\
        {Val. folds Min DONE} & {0.13-0.28}  & {0.09-0.11} & {0.35-0.87} & {0.19-0.25} & {0.2-0.2} \\
        \hline
        Test (QT) DONE & 0.3295 & 0.1452 & 0.7740 & 0.2644 & 0.1463 \\
        \hline
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Calibrated LApredict QT and OPENSTACK}
    \label{calibrated_LApredict}
\end{table}

==> tables/uncalibrated_CodeBERT4JIT.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
                \multicolumn{6}{|c|}{CodeBERT4JIT with OPENSTACK} \\
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} & {0.3038} & {0.111} & {0.7189} & {0.4378}  & {0.1237} \\ 
        {Val. Min-Max} & 0.20-0.43  & 0.08-0.15 & 0.50-0.91 & 0.21-0.73 & 0.10-0.15 \\
        \rowcolor[HTML]{EFEFEF}         \hline
        Test & 0.2896 & 0.1106 & 0.6993 & 0.4325 & 0.1242 \\
                \hline
        \multicolumn{6}{|c|}{CodeBERT4JIT with QT}\\
        \hline
                \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} &  0.358 &   0.0667 &  0.8185 &  0.3056 &  0.0766 \\
        {Val. folds Min} &  0.23-0.46 & 0.04-0.11 & 0.60-0.98 &  0.11-0.73 & 0.05-0.11 \\
        \rowcolor[HTML]{EFEFEF} 
        \hline
        Test & 0.3098 & 0.0667 & 0.7423 & 0.3078 & 0.0759 \\
        \hline
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Original CodeBERT4JIT calibration scores}
        \label{uncalibrated_CodeBERT}
\end{table}


==> tables/uncalibrated_DeepJIT.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
        \multicolumn{6}{|c|}{DeepJIT with OPENSTACK}\\
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} & {0.3509} & {0.3509} & {0.6197} & {0.5302}  & {0.2378} \\ 
        {Val. Min-Max} & 0.32-0.37  & 0.32-0.37 & 0.52-0.87 & 0.49-0.57 & 0.21-0.25 \\
        \rowcolor[HTML]{EFEFEF} 
        \hline
        Test & 0.3470 & 0.3470 & 0.5820 & 0.5628 & 0.2362 \\
        \hline
        \multicolumn{6}{|c|}{DeepJIT with QT}\\
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} & 0.3330 &   0.3330 &  0.6177 & 0.5784 &  0.1923\\
        {Val. Min-Max} & 0.31-0.35 & 0.31-0.35 & 0.58-0.69 & 0.53-0.62 & 0.18-0.21 \\
        \rowcolor[HTML]{EFEFEF} 
        \hline
        Test & 0.3264 & 0.3264 & 0.6633 & 0.6168 & 0.1927 \\
        \hline  
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Original DeepJIT calibration scores}
    \label{uncalibrated_deepJIT}
\end{table}







==> tables/uncalibrated_LApredict.tex <==
\begin{table}[h!]
    \centering    
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \rowcolor[HTML]{EFEFEF} 
        \textbf{Data subset} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \textbf{Brier} \\
        & Equidistant & Equisized & Equidistant & Equisized & \\
        \rowcolor[HTML]{EFEFEF} 
        & 15 bins & 15 bins & 15 bins & 15 bins &  \\
        \hline
        \multicolumn{6}{|c|}{LApredict with OPENSTACK}\\
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} & {0.2260} & {0.1039} & {0.5768} & {0.2197} & {0.1910} \\ 
        {Val. Min-Max} & 0.15-0.30  & 0.09-0.11 & 0.35-0.93 & 0.18-0.24 & 0.19-0.2 \\
        \rowcolor[HTML]{EFEFEF} 
        \hline
        Test & 0.1298 & 0.0911 & 0.3929 & 0.2126 & 0.1492 \\
        \hline
        \multicolumn{6}{|c|}{LApredict with QT}\\
        \hline
        \rowcolor[HTML]{EFEFEF} 
        {Val. folds Avg} & 0.1927 &   0.1034 & 0.4585 & 0.2126 & 0.2051 \\
        {Val. Min-Max} & 0.13-0.24 & 0.09-0.11 & 0.29-0.58 & 0.2-0.26 & 0.2-0.21 \\
        \rowcolor[HTML]{EFEFEF} 
        \hline
        Test & 0.2978 & 0.1433 & 0.8259 & 0.2626 & 0.1460 \\
        \hline  
    \end{tabular}
    \vspace{0.3mm} 
    \caption{Original LApredict calibration scores (without calibration)}
    \label{uncalibrated_LApredict}
\end{table}
